VersatileMotion: A Unified Framework for Motion Synthesis and Comprehension

Large language models (LLMs) are, by design, inherently capable of multi-task learning: through a unified next-token prediction paradigm, they can naturally address a wide variety of downstream tasks. Prior work in the motion domain has demonstrated some generality by adapting LLMs via a Motion Tokenizer coupled with an autoregressive Transformer to generate and understand human motion. However, this generality remains limited in scope and yields only modest performance gains. We introduce VersatileMotion, a unified multimodal motion LLM that combines a novel motion tokenizer, integrating VQ-VAE with flow matching, and an autoregressive transformer backbone to seamlessly support at least nine distinct motion-related tasks. VersatileMotion is the first method to handle single-agent and multi-agent motions in a single framework and enable cross-modal conversion between motion, text, music, and speech, achieving state-of-the-art performance on seven of these tasks. Each sequence in MotionHub may include one or more of the following annotations: natural-language captions, music or audio clips, speech transcripts, and multi-agent interaction data. To facilitate evaluation, we define and release benchmark splits covering nine core tasks. Extensive experiments demonstrate the superior performance, versatility, and potential of VersatileMotion as a foundational model for future understanding and generation of motion.

==> depds/tab_abl_in_act_out_norm.tex <==
\begin{table*}
    \centering
    \caption{Comparison of the effects of different input activation and output normalization.}
    \adjustbox{width=0.9\linewidth}{
    \begin{tabular}{ll|ccc|ccc|cc}
    
    \toprule 
     \multirow{2}{*}{\centering Norm} & \multirow{2}{*}{\centering Act} & \multicolumn{3}{c|}{MPJPE} & \multicolumn{3}{c|}{PA-MPJPE} & \multirow{2}{*}{\centering ADE} & \multirow{2}{*}{\centering FDE}\\
     & & all & body & hand & all & body & hand & & \\
    \midrule

    \checkmark & $\times$ & - & - & - & - & - & - & - & - \\
    \checkmark & \checkmark & 0.0751 & 0.0723 & 0.0773 & 0.0474 & 0.0557 & 0.0406 & 0.0073 & 0.0093 \\
    $\times$ & \checkmark & 0.0757 & 0.0725 & 0.0783 & 0.0477 & 0.0564 & 0.0407 & 0.0064 & 0.0091 \\
    $\times$ & $\times$ & 0.0726 & 0.0695 & 0.0751 & 0.0454 & 0.0537 & 0.0388 & 0.0056 & 0.0080 \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:abl_in_act_out_norm}
\end{table*}


==> depds/tab_abl_mid_layer.tex <==
\begin{table*}
    \centering
    \caption{Comparison of reconstruction performance with and without mid layers.}
    \adjustbox{width=0.9\linewidth}{
    \begin{tabular}{l|ccc|ccc|cc}
    
    \toprule 
     Metrics & \multicolumn{3}{c|}{MPJPE} & \multicolumn{3}{c|}{PA-MPJPE} & \multirow{2}{*}{\centering ADE} & \multirow{2}{*}{\centering FDE}\\
    Mid Layer & all & body & hand & all & body & hand & & \\
    \midrule
    $\times$ & 0.0902 & 0.0861 & 0.0933 & 0.0531 & 0.0626 & 0.0461 & 0.0085 & 0.0109 \\ 
    \checkmark & 0.0800 & 0.0765 & 0.0828 & 0.0494 & 0.0581 & 0.0423 & 0.0066 & 0.0099 \\ 


    \bottomrule
    \end{tabular}
    }
    \label{tab:abl_mid_layer}
\end{table*}


==> depds/tab_abl_num_layers.tex <==
\begin{table*}
    \centering
    \caption{Reconstruction metrics of Motion VQ-VAE with different num layers.}
    \adjustbox{width=0.9\linewidth}{
    \begin{tabular}{l|ccc|ccc|cc}
    
    \toprule 
     Metrics & \multicolumn{3}{c|}{MPJPE} & \multicolumn{3}{c|}{PA-MPJPE} & \multirow{2}{*}{\centering ADE} & \multirow{2}{*}{\centering FDE}\\
    Layers & all & body & hand & all & body & hand & & \\
    \midrule
    2 & - & - & - & - & - & - & - & - \\ 
    3(down first) & 0.1818 & 0.1651 & 0.1954 & 0.0866 & 0.1000 & 0.0757 & 0.0183 & 0.0221 \\ 
    3(down post) & 0.1724 & 0.1548 & 0.1865 & 0.0859 & 0.0996 & 0.0748 & 0.0162 & 0.0193 \\ 
    4 & - & - & - & - & - & - & - & - \\ 


    \bottomrule
    \end{tabular}
    }
    \label{tab:abl_nlayers}
\end{table*}


==> depds/tab_abl_updown_type.tex <==
\begin{table*}
    \centering
    \caption{Reconstruction metrics of Motion VQ-VAE with different depths.}
    \adjustbox{width=0.9\linewidth}{
    \begin{tabular}{l|ccc|ccc|cc}
    
    \toprule 
     Metrics & \multicolumn{3}{c|}{MPJPE} & \multicolumn{3}{c|}{PA-MPJPE} & \multirow{2}{*}{\centering ADE} & \multirow{2}{*}{\centering FDE}\\
    Dilation & all & body & hand & all & body & hand & & \\
    \midrule
    vanilla & 0.1888 & 0.1768 & 0.1984 & 0.0874 & 0.1023 & 0.0754 & 0.0192 & 0.0205 \\
    hybrid & 0.1924 & 0.1780 & 0.2039 & 0.0907 & 0.1050 & 0.0791 & 0.0190 & 0.0205 \\


    \bottomrule
    \end{tabular}
    }
    \label{tab:abl_updown_type}
\end{table*}

